Towards S-NAMO: Socially-aware Navigation Among Movable Obstacles

In this paper, we present an in-depth analysis of Navigation Among Movable Obstacles (NAMO) literature, notably highlighting that social acceptability remains an unadressed problem in this robotics navigation domain. The objectives of a Socially-Aware NAMO are defined and a first set of algorithmic propositions is built upon existing work. We developed a simulator allowing to test our propositions of social movability evaluation for obstacle selection, and social placement of objects with a semantic map layer. Preliminary pushing tests are done with a Pepper robot, the standard platform for the Robocup@home Social Standard Platform League, in the context of our participation (LyonTech Team).

==> Algorithms/01-wu-optevaluateaction.tex <==
\begin{algorithm}[H]

  \caption{Optimized algorithm for NAMO in unknown environments of Wu et. al. (2010), fixed - ACTION EVALUATION SUBROUTINE}

  \label{alg:01-wu-optevaluateaction}

  \begin{algorithmic}[1]

    \Procedure{OPT-EVALUATE-ACTION}{$o$, $d$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$}

      \If{$o \in blockedObsL$}
        \State \textbf{return} null
      \EndIf

      \State $P_{o,d} \gets \emptyset$
      \State $c_{1} \gets A$*($R$, $o.init$, $I.occGrid$) \label{lst:line:obstacle_pushpose_note}
      \If{$c_{1} = \emptyset$} \label{lst:line:c1_note}
        \State \textbf{return} null
      \EndIf
      \State $c_{2} \gets \emptyset$
      \State $oSimPose \gets o.init$

      \While{push on $o$ in $d$ possible AND $|c_{2}| * pushCost \leq p_{opt}.cost$} \label{lst:line:bound_note}
        \State $oSimPose \gets oSimPose + one\_push\_in\_d$
        \If{push created new opening}
          \State $c_{2} \gets \{o.init, oSimPose\}$ \label{lst:line:c2_note}
          \State $c_{3} \gets A$*($oSimPose$, $R_{goal}$, $I.withSimulatedObstacleMove$)
          \If{$c_{3} \neq \emptyset$} \label{lst:line:c3_note}
            \State $p.components \gets$ [$c_{1}$, $c_{2}$, $c_{3}$]
            \State $p.cost \gets (|c_{1}| + |c_{3}|) * moveCost + |c_{2}| * pushCost$
            \State $p.minCost \gets |c_{2}| * pushCost + |c_{3}| * moveCost$
            \State $p.o, p.d \gets o, d$
            \State $P_{o,d} \gets P_{o,d} \bigcup \{p\}$
          \EndIf
        \EndIf
      \EndWhile

      \State \textbf{return} $p \in P_{o,d}$ with minimal $p.cost$ or null if $P_{o,d} = \emptyset$

    \EndProcedure

  \end{algorithmic}

\end{algorithm}


==> Algorithms/01-wu-optimized.tex <==
\begin{algorithm}[H]

  \caption{Optimized algorithm for NAMO in unknown environments of Wu et. al. (2010), fixed - MAIN LOOP}

  \label{alg:01-wu-optimized-part1}

  \begin{algorithmic}[1]

      \Procedure{OPTIMIZED}{$R_{init}$, $R_{goal}$}

        \State $R \gets R_{init}$ \label{lst:line:01_plan_execution_loop_1}

        \State $blockedObsL \gets \emptyset$

        \State $P_{sort} \gets \emptyset$

        \State $\mathcal{O}_{new} \gets \emptyset$

        \State $isManipSuccess \gets True$

        \State $I \gets empty\_occupation\_grid$

        \State $p_{opt}.components \gets$ [$A$*($R_{init}$, $R_{goal}$, $I.occGrid$)]

        \State $p_{opt}.cost \gets |p_{opt}.components[0]| * moveCost$

        \While{$R \neq R_{goal}$}

          \State UPDATE-FROM-NEW-INFORMATION($I$)\label{lst:line:update-from-new-information_note}

          \State $\mathcal{O}_{new} \gets \mathcal{O}_{new} \bigcup I.newObstacles$

          \State $isPlanNotColliding \gets p_{opt} \bigcap \mathcal{O}_{new} \neq \emptyset$ \label{lst:line:intersection_note}

          \If{\textbf{not}($isPlanNotColliding$ AND $isManipSuccess$)}

            \State $p_{opt}.components \gets$ [$A$*($R$, $R_{goal}$, $I.occGrid$)]
            \State $p_{opt}.cost \gets |p_{opt}.components[0]| * moveCost$ \label{lst:line:01_plan_execution_loop_2}

            \For{each $o \in \mathcal{O}_{new}$} \label{lst:line:01_obstacle evaluation_loop_1}
              \For{each possible push direction $d$ on $o$}
                \State $p \gets$ OPT-EVALUATE-ACTION($o$, $d$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$)
                \If{$p \neq$ null}
                  \State $P_{sort}$.insert(p)
                \EndIf
              \EndFor
            \EndFor

            \If{$P_{sort} \neq \emptyset$}
              \State $p_{next} \gets P_{sort}[0]$
              \While{$p_{opt}.cost \geq p_{next}.minCost$ AND $p_{next} \neq$ null}
                \State $p \gets$ OPT-EVALUATE-ACTION($p_{next}.o$, $p_{next}.d$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$) \label{lst:line:suppcondition}
                \If{$p \neq$ null AND $p.cost \leq p_{opt}.cost$}
                  \State $p_{opt} \gets p$
                \EndIf
                \State $p_{next} \gets P_{sort}$.getNext()
              \EndWhile
            \EndIf \label{lst:line:01_obstacle evaluation_loop_2}

            \algstore{wustore}

  \end{algorithmic}

\end{algorithm}

\begin{algorithm}[H]

  \label{alg:01-wu-optimized-part2}

  \begin{algorithmic}[1]

            \algrestore{wustore}

            \State $\mathcal{O}_{new} \gets \emptyset$ \label{lst:line:01_plan_execution_loop_3}

          \EndIf
          \If{$p_{opt}.components = \emptyset$} \label{lst:line:stop_condition_note}
            \State \textbf{return} $False$
          \EndIf

          \State $isManipSuccess \gets True$ \label{lst:line:plan_following_note_1}
          \State $R_{next} \gets p_{opt}$.getNextStep()
          \State $R_{real} \gets$ ROBOT-GOTO($R_{next}$)
          \If{$p_{opt}.nextStepComponent$ is $c_{2}$ AND $R_{real} \neq R_{next}$}
            \State $isManipSuccess \gets False$
            \State $blockedObsL \gets blockedObsL \bigcup p_{opt}.o$
          \EndIf
          \State $R \gets R_{real}$ \label{lst:line:plan_following_note_2}

        \EndWhile

        \State \textbf{return} $True$ \label{lst:line:01_plan_execution_loop_4}

    \EndProcedure

  \end{algorithmic}

\end{algorithm}


==> Algorithms/02-levihn-makeandexecuteplan.tex <==
\begin{algorithm}[H]

  \caption{Optimized algorithm for NAMO in unknown environments of Wu et. al. adapted according to M.Levihn et. al.'s (2014) recommandations - EXECUTION LOOP}

  \label{alg:02-levihn-makeandexecuteplan}

  \begin{algorithmic}[1]

    \Procedure{MAKE-AND-EXECUTE-PLAN}{$R_{init}$, $R_{goal}$}

      \State $R \gets R_{init}$ \label{lst:line:init1}
      \State $\mathcal{O}_{new} \gets \emptyset$
      \State $isManipSuccess \gets True$
      \State $blockedObsL \gets \emptyset$
      \State $euCostL, minCostL \gets \emptyset, \emptyset$ \label{lst:line:init2}
      \State $I \gets empty\_occupation\_grid$
      \State $p_{opt}.components \gets [D$*Lite($R_{init}$, $R_{goal}$, $I.occGrid$)]
      \State $p_{opt}.cost \gets |p_{opt}| * moveCost$

      \While{$R \neq R_{goal}$}

        \State UPDATE-FROM-NEW-INFORMATION($I$)

        \If{$I$.freeSpaceCreated()} \label{lst:line:second_update-from-new-information_note}
          \State $minCostL \gets \emptyset$
        \EndIf

        \State $\mathcal{O}_{new} \gets \mathcal{O}_{new} \bigcup I.newObstacles$

        \State $\mathcal{O} \gets I.allObstacles$ \label{lst:line:allobstacles}

        \State $isPlanNotColliding \gets p_{opt} \bigcap \mathcal{O}_{new} \neq \emptyset$

        \If{\textbf{not}($isPlanNotColliding$ AND $isManipSuccess$)}
          \State $p_{opt}.components \gets [D$*Lite($R$, $R_{goal}$, $I.occGrid$)]
          \State $p_{opt}.cost \gets |p_{opt}| * moveCost$
          \State MAKE-PLAN($R$, $R_{goal}$, $I$, $\mathcal{O}$, $blockedObsL$, $p_{opt}$, $euCostL$, $minCostL$)
          \State $\mathcal{O}_{new} \gets \emptyset$
        \EndIf

        \If{$p_{opt}.components = \emptyset$} \label{lst:line:exec1}
          \State \textbf{return} $False$
        \EndIf \label{lst:line:exec1bis}

        \State $isManipSuccess \gets True$ \label{lst:line:ismanipsuccess}
        \State $R_{next} \gets p_{opt}$.getNextStep() \label{lst:line:exec2bis}
        \State $R_{real} \gets$ ROBOT-GOTO($R_{next}$)
        \If{$p_{opt}.nextStepComponent$ is $c_{2}$ AND $R_{real} \neq R_{next}$}
          \State $isManipSuccess \gets False$
          \State $blockedObsL \gets blockedObsL \bigcup p_{opt}.o$
        \EndIf
        \State $R \gets R_{real}$ \label{lst:line:exec2}

      \EndWhile

      \State \textbf{return} $True$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/02-levihn-makeplan.tex <==
\begin{algorithm}[H]

  \caption{Optimized algorithm for NAMO in unknown environments of Wu et. al. adapted according to M.Levihn et. al.'s (2014) recommandations - PLAN COMPUTATION}

  \label{alg:02-levihn-makeplan}

  \begin{algorithmic}[1]

    \Procedure{MAKE-PLAN}{$R$, $R_{goal}$, $I$, $\mathcal{O}$, $blockedObsL$, $p_{opt}$, $euCostL$, $minCostL$}

      \For{each $o \in \mathcal{O}$}
          \State $C_{3_{(Est)}} \gets \min(\{\forall graspPoint \in o.graspPoints \hspace{0.2cm} || \hspace{0.2cm} |\{graspPoint, R_{goal}\}|\})$
          \State $euCostL$.insertOrUpdate$(\{o, C_{3_{(Est)}}\})$
      \EndFor

      \State $i_{e}, i_{m} \gets 0 , 0$
      \State $evaluatedObstacles \gets \emptyset$ \label{lst:line:evaluated_obstacles_note_1}

      \While{$\min(minCostL[i_{m}].minCost, euCostL[i_{e}].c_{3_{est}}) < p_{opt}.cost$} \label{lst:line:stop_condition_obs_loop}
        \If{$minCostL[i_{m}].minCost < euCostL[i_{e}].c_{3_{est}}$} \label{lst:line:mincostl_first}
          \State $o \gets minCostL[i_{m}].obstacle$
          \If{$o \not\in evaluatedObstacles$} \label{lst:line:evaluated_obstacles_note_2}
            \State $p \gets$ PLAN-FOR-OBSTACLE($o$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$)
            \If{$p \neq$ null}
              \State $minCostL.$insertOrUpdate$(\{o, p.minCost\})$
            \Else
              \State $minCostL.$insertOrUpdate$(\{o, +\infty\})$
            \EndIf
            \State $evaluatedObstacles.$insert$(o)$ \label{lst:line:evaluated_obstacles_note_3}
          \EndIf
          \State $i_{m} \gets i_{m} + 1$
        \Else
          \If{not $minCostL$.contains($euCostL[i_{e}].obstacle)$} \label{lst:line:use_eucostl_1}
          \State $o \gets euCostL[i_{e}].obstacle$
            \If{$o \not\in evaluatedObstacles$} \label{lst:line:evaluated_obstacles_note_4}
              \State $p \gets$ PLAN-FOR-OBSTACLE($o$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$)
              \If{$p \neq$ null}
                \State $minCostL.$insertOrUpdate$(\{o, p.minCost\})$
              \Else
                \State $minCostL.$insertOrUpdate$(\{o, +\infty\})$
              \EndIf
              \State $evaluatedObstacles.$insert$(o)$ \label{lst:line:evaluated_obstacles_note_5}
            \EndIf
          \EndIf
          \State $i_{e} \gets i_{e} + 1$ \label{lst:line:use_eucostl_2}
        \EndIf
      \EndWhile
    \EndProcedure
  \end{algorithmic}
\end{algorithm}


==> Algorithms/02-levihn-planforobstacle.tex <==
\begin{algorithm}[H]

  \caption{Optimized algorithm for NAMO in unknown environments of Wu et. al. adapted according to M.Levihn et. al.'s (2014) recommandations - PLAN EVALUATION FOR A SINGLE OBSTACLE}

  \label{alg:02-levihn-planforobstacle}

  \begin{algorithmic}[1]

    \Procedure{PLAN-FOR-OBSTACLE}{$o$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$}

      \If{$o \in blockedObsL$}
        \State \textbf{return} null
      \EndIf

      \State $P_{o,d}$ $\gets \emptyset$
      \State $c_{1} \gets D$*Lite$(R, o.init, I)$
      \If{$c_{1} = \emptyset$}
        \State \textbf{return} null
      \EndIf
      \State $BA \gets null$ \label{lst:line:remember_ba_note_1}

      \For{each possible manipulation direction $d$ on $o$}

        \State $seq \gets 1$

        \State $oSimPose \gets o.init + one\_translation\_in\_d$

        \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$ \label{lst:line:new_bound_1}

        \State $C_{est} \gets (|c_{1}| + |c_{3_{(Est)}}|) * moveCost + seq * |one\_translation\_in\_d| * pushCost$

        \While{$C_{est}$ $ \leq p_{opt}.cost$ AND manipulation on $o$ possible} \label{lst:line:new_bound_2}

          \If{CHECK-NEW-OPENING($I.occGrid$, $o$, $seq * one\_translation\_in\_d$, $BA$)} \label{lst:line:remember_ba_note_2}
            \State $c_{2} \gets \{o.init, oSimPose\}$
            \State $c_{3} \gets D$*Lite($oSimPose$, $R_{goal}$, $I.withSimulatedObstacleMove$)
            \If{$c_{3} \neq \emptyset$}
              \State $p.components \gets$ [$c_{1}$, $c_{2}$, $c_{3}$]
              \State $p.cost \gets (|c_{1}| + |c_{3}|) * moveCost + |c_{2}| * pushCost$
              \State $p.minCost \gets |c_{2}| * pushCost + |c_{3}| * moveCost$
              \State $p.o, p.d \gets o, d$
              \State $P_{o,d} \gets P_{o,d} \bigcup \{p\}$
              \If{$p.cost < p_{opt}.cost$}
                \State $p_{opt} \gets p$
              \EndIf
            \EndIf
          \EndIf

          \State $seq \gets seq + 1$

          \State $oSimPose \gets oSimPose + one\_translation\_in\_d$

          \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$

          \State $C_{est} \gets (|c_{1}| + |c_{3_{(Est)}}|) * moveCost + seq * |one\_translation\_in\_d| * pushCost$

        \EndWhile

      \EndFor

    \State \textbf{return} $p \in P_{o,d}$ with minimal $p.cost$ or null if $P_{o,d} = \emptyset$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/03-custom-basicmods-makeandexecuteplan.tex <==
\begin{algorithm}[H]

  \caption{Execution loop taking our hypotheses into account.}

  \label{alg:03-custom-basicmods-makeandexecuteplan}

  \begin{algorithmic}[1]

    \Procedure{MAKE-AND-EXECUTE-PLAN}{$R_{init}$, $R_{goal}$, $I_{init}$} \label{lst:line:partialline_1}

      \State \dots \label{lst:line:initbis1} \Comment{Initialization (lines \ref{lst:line:init1} to \ref{lst:line:init2} in Algorithm \ref{alg:02-levihn-makeandexecuteplan})}

      \State \hlgreen{$I \gets I_{init}$} \label{lst:line:partialline_2}

      \State $p_{opt}.components \gets [$\hlgreen{$A$*}($R_{init}$, $R_{goal}$, $I.occGrid$)]
      \State $p_{opt}.cost \gets |p_{opt}| * moveCost$ \label{lst:line:initbis2}

      \While{$R \neq R_{goal}$}

        \State UPDATE-FROM-NEW-INFORMATION($I$) \label{lst:line:knowledge1}

        \If{$I$.freeSpaceCreated}
          \State $minCostL \gets \emptyset$
        \EndIf

        \State $\mathcal{O}_{new} \gets \mathcal{O}_{new} \bigcup I.newObstacles$

        \State $\mathcal{O} \gets I.allObstacles$

        \State $isPlanNotColliding \gets p_{opt} \bigcap \mathcal{O}_{new} \neq \emptyset$

        \State \hlgreen{$isPushPoseValid \gets True$} \label{lst:line:validity1}
        \State \hlgreen{$isManipSafe \gets True$}
        \State \hlgreen{$isObstacleSame \gets True$}
        \If{\hlgreen{$p_{opt}.o$ exists}} \Comment{If $p_{opt}$ includes the manipulation of an obstacle.} \label{lst:line:checkvalidity_1}
          \State \hlgreen{$isObstacleSame \gets \mathcal{O}[p_{opt}.o] = p_{opt}.o$} \label{lst:line:brackets_operator_1}
          \If{\hlgreen{\textbf{not} $isObstacleSame$}}
            \State \hlgreen{$p_{opt}.o \gets \mathcal{O}[p_{opt}.o.id]$} \Comment{Update the copy.} \label{lst:line:brackets_operator_2}
            \State \hlgreen{$p_{opt}.safeSweptArea \gets$ GET-SAFE-SWEPT-AREA($p_{opt}.o$, $p_{opt}.translation$, $I$)} \label{lst:line:get_safe_swept_are_call_1}
            \If{\hlgreen{$p_{opt}.nextStepComponent$ is $ c_{1}$ AND $p_{opt}.pushPose \not\in p_{opt}.o.pushPoses$}} \label{lst:line:pushpose_1}
              \State \hlgreen{$isPushPoseValid \gets False$}
            \EndIf \label{lst:line:pushpose_2}
          \EndIf
          \If{\hlgreen{$p_{opt}.safeSweptArea \bigcap \mathcal{O} \neq \emptyset$}} \label{lst:line:area_intersect_1}
            \State \hlgreen{$isManipSafe \gets False$}
          \EndIf \label{lst:line:area_intersect_2}
        \EndIf \label{lst:line:knowledge2} \label{lst:line:validity2}

        \If{\textbf{not}($isPlanNotColliding$ AND $isManipSuccess$ \hlgreen{AND $isManipSafe$ AND $isPushPoseValid$})}
          \State $p_{opt}.components \gets$ [\hlgreen{$A$*}($R$, $R_{goal}$, $I.occGrid$)]
          \State $p_{opt}.cost \gets |p_{opt}| * moveCost$
          \State MAKE-PLAN($R$, $R_{goal}$, $I$, $\mathcal{O}$, $blockedObsL$, $p_{opt}$, $euCostL$, $minCostL$)
          \State $\mathcal{O}_{new} \gets \emptyset$
        \EndIf

        \State \dots \Comment{Execution (lines \ref{lst:line:exec1} to \ref{lst:line:exec2} in Algorithm \ref{alg:02-levihn-makeandexecuteplan})}

      \EndWhile

      \State \textbf{return} $True$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/03-custom-basicmods-planforobstacle.tex <==
\begin{algorithm}[H]

  \caption{Obstacle evaluation subroutine taking our hypotheses into account.}

  \label{alg:03-custom-basicmods-planforobstacle}

  \begin{algorithmic}[1]

    \Procedure{PLAN-FOR-OBSTACLE}{$o$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$}

      \If{$o \in blockedObsL$} \label{lst:line:initobs1}
        \State \textbf{return} null
      \EndIf \label{lst:line:initobs2}

      \State $P_{o,d}$ $\gets \emptyset$
      % \State $BA \gets null$

      \For{\hlgreen{each $pushPose$ in $o.pushPoses$}}
        \State \hlgreen{$pushUnit \gets (cos(pushPose.yaw), sin(pushPose.yaw))$} \label{lst:line:loop1} \Comment{Unit vector for push direction}

        \State \hlgreen{$c_{1} \gets A$*($R$, $pushPose$, $I.occGrid$)} \Comment{$c_{1}$ is computed for each push pose}

        \If{$c_{1} = \emptyset$}
          \State \hlgreen{\textbf{continue}} \label{lst:line:continue_note}
        \EndIf

        \State $seq \gets 1$

        \State \hlgreen{$translation \gets pushUnit * onePushDist * seq$} \Comment{onePushDist is a distance constant}

        \State \hlgreen{$safeSweptArea \gets $GET-SAFE-SWEPT-AREA($o$, $translation$, $I.occGrid$)}

        \State $oSimPose \gets $\hlgreen{$pushPose + translation$} \label{lst:line:loop2}

        \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$

        \State $C_{est} \gets (|c_{1}| + |c_{3_{(Est)}}|) * moveCost + $\hlgreen{$|translation| * o.pushCost$}

        \While{$C_{est}$ $ \leq p_{opt}.cost$ AND \hlgreen{$safeSweptArea \neq$ null}}

          % \If{CHECK-NEW-OPENING($I.occGrid$, $o$, $translation$, $BA$)}
            \State $c_{2} \gets \{$\hlgreen{$pushPose$}$, oSimPose\}$
            \State \hlgreen{$c_{3} \gets A$*($oSimPose$, $R_{goal}$, $I.withSimulatedObstacleMove$)}
            \If{$c_{3} \neq \emptyset$}
              \State $p.components \gets$ [$c_{1}$, $c_{2}$, $c_{3}$]
              \State $p.cost \gets (|c_{1}| + |c_{3}|) * moveCost + |c_{2}| * $\hlgreen{$o.pushCost$}
              \State $p.minCost \gets |c_{2}| * $\hlgreen{$o.pushCost$}$ + |c_{3}| * moveCost$
              \State $p.o \gets$ \hlgreen{COPY($o$)} \label{lst:line:ovaraffec1} \label{lst:line:copy_note}
              \State \hlgreen{$p.translation \gets translation$}
              \State \hlgreen{$p.safeSweptArea \gets safeSweptArea$}
              \State \hlgreen{$p.pushPose \gets pushPose$}
              \State $P_{o,d} \gets P_{o,d} \bigcup \{p\}$
              \If{$p.cost < p_{opt}.cost$}
                \State $p_{opt} \gets p$
              \EndIf \label{lst:line:ovaraffec2}
            \EndIf
          % \EndIf

          \State $seq \gets seq + 1$ \label{lst:line:loopvarup1}

          \State \hlgreen{$translation \gets pushUnit * onePushDist * seq$}

          \State \hlgreen{$safeSweptArea \gets $GET-SAFE-SWEPT-AREA($o$, $translation$, $I$)} \label{lst:line:get_safe_swept_are_call_2}

          \State $oSimPose \gets $\hlgreen{$pushPose + translation$} \label{lst:line:loopvarup2}

          \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$

          \State $C_{est} \gets (|c_{1}| + |c_{3_{(Est)}}|) * moveCost + $\hlgreen{$|translation| * o.pushCost$}

        \EndWhile

      \EndFor

    \State \textbf{return} $p \in P_{o,d}$ with minimal $p.cost$ or null if $P_{o,d} = \emptyset$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/04-custom-observation-makeandexecuteplan.tex <==
\begin{algorithm}[H]

  \caption{Execution loop modified for allowing observation.}

  \label{alg:04-custom-observation-makeandexecuteplan}

  \begin{algorithmic}[1]

    \Procedure{MAKE-AND-EXECUTE-PLAN}{$R_{init}$, $R_{goal}$, $I_{init}$}

      \State \dots \Comment{Initialization (lines \ref{lst:line:initbis1} to \ref{lst:line:initbis2} in Algorithm \ref{alg:03-custom-basicmods-makeandexecuteplan})}

      \State \hlgreen{$isObservable \gets True$}

      \While{$R \neq R_{goal}$}

        \State UPDATE-FROM-NEW-INFORMATION($I$)

        \State \dots \Comment{Knowledge update and checks (lines \ref{lst:line:knowledge1} to \ref{lst:line:knowledge2} in Algorithm \ref{alg:03-custom-basicmods-makeandexecuteplan})}

        \If{\textbf{not}($isPlanNotColliding$ AND $isManipSuccess$ AND $isManipSafe$ AND $isPushPoseValid$ \hlgreen{AND $isObservable$})}
          \State $p_{opt}.components \gets [A$*($R$, $R_{goal}$, $I.occGrid$)]
          \State $p_{opt}.cost \gets |p_{opt}| * moveCost$
          \State MAKE-PLAN($R$, $R_{goal}$, $I$, $\mathcal{O}$, $blockedObsL$, $p_{opt}$, $euCostL$, $minCostL$)
          \State $\mathcal{O}_{new} \gets \emptyset$
        \EndIf

        \If{$p_{opt}.components = \emptyset$}
          \State \textbf{return} $False$
        \EndIf

        \State $isManipSuccess \gets True$
        \State \hlgreen{$isObservable \gets True$}
        \State $R_{next} \gets p_{opt}$.getNextStep()
        \If{\hlgreen{$p_{opt}.o \neq$ null $p_{opt}.o.movableStatus = IS\_MAYBE\_MOVABLE$ AND \textbf{not} $isObstacleSame$ AND ($c_{next} = c_{0}$ OR $c_{next} = c_{1}$)}}
          \State \hlgreen{$fObsPose \gets$ GET-FIRST-PATH-OBSPOSE($p_{opt}.o$, $p_{opt}$.get-$c_{0}$() + $p_{opt}$.get-$c_{1}$(), $I$)}
          \If{\hlgreen{$fObsPose =$ null}}
            \State \hlgreen{$isObservable \gets False$}
            \State \hlgreen{\textbf{continue}}
          \EndIf
        \EndIf
        \State $R_{real} \gets$ ROBOT-GOTO($R_{next}$)
        \If{$p_{opt}.nextStepComponent$ is $c_{2}$ AND $R_{real} \neq R_{next}$}
          \State $isManipSuccess \gets False$
          \State $blockedObsL \gets blockedObsL \bigcup p_{opt}.o$
        \EndIf
        \State $R \gets R_{real}$

      \EndWhile

      \State \textbf{return} $True$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/04-custom-observation-optimized-compute01c1.tex <==
\begin{algorithm}[H]

  \caption{Optimized subroutine for computing $c_{0}$ and $c_{1}$ if $c_{1}$ is not already valid.}

  \label{alg:04-custom-observation-optimized-compute01c1}

  \begin{algorithmic}[1]

    \Procedure{OPT-COMPUTE-C0-C1}{$o$, $I$, $R$, $pushPose$, $c_{0}$, $c_{1}$}
      \State $c_{1} \gets \emptyset$
      \State $totalCost \gets +\infty$

      %   % The computation time could be reduced by computing the heuristic
      %   % euclidean cost from current position to obstacle only once and not
      %   % as many times as there are push poses for the obstacle.
      %   % This needs to be added to the calling method and euCostToObsL passed in parameter.
      % \If{$o.movableStatus = IS\_MAYBE\_MOVABLE$}
      %   \State $euCostToObsL \gets \emptyset$
      %   \For{each $obsPose$ in $o.obsPoses$}
      %     \State $euCostToObsL$.insert$(\{obsPose, |{R, obsPose}|\})$
      %   \EndFor
      %
      % \EndIf

      \State $euPosesCostL \gets \emptyset$ \Comment{Sort observation poses by ascending heuristic cost.} \label{lst:line:occ_heur_1}
      \For{each $obsPose$ in $o.obsPoses$}
        \State $euPosesCostL$.insert$(\{obsPose, |{R, obsPose}| + |{obsPose, pushPose}|\})$
      \EndFor \label{lst:line:occ_heur_2}

      \If{$euPosesCostL \neq \emptyset$} \label{lst:line:traverse_eu_1}
        \State $op_{next} \gets euPosesCostL[0]$
        \While{$totalCost \geq op_{next}.cost$ AND $op_{next} \neq$ null}
          \State $c_{0_{cur}} \gets A$*($R$, $op_{next}.obsPose$, $I.occGrid$)
          \State $c_{1_{cur}} \gets A$*($op_{next}.obsPose$, $pushPose$, $I.occGrid$)
          \State $newTotalCost = |c_{0_{cur}}| + |c_{1_{cur}}|$
          \If{$newTotalCost < +\infty$ AND ($newTotalCost < totalCost$ OR ($newTotalCost = totalCost$ AND $|c_{0_{cur}}| < |c_{0}|$)}
            \State $c_{0} = c_{0_{cur}}$
            \State $c_{1} = c_{1_{cur}}$
            \State $totalCost = |c_{0}| + |c_{1}|$
          \EndIf
          \State $op_{next} \gets euPosesCostL$.getNext()
        \EndWhile
      \EndIf \label{lst:line:traverse_eu_2}
    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/04-custom-observation-simple-checkpath.tex <==
\begin{algorithm}[H]

  \caption{Subroutine for getting the first pose in a $path$ that allows identification of $o$, it it exists.}

  \label{alg:04-custom-observation-simple-checkpath}
  
  \begin{algorithmic}[1]

    \Procedure{GET-FIRST-PATH-OBSPOSE}{$o$, $path$, $I$}
      \For{each $pose$ in $path$}
        \If{IS-OBS-IN-FOV-FOR-POSE($o$, $pose$, $I$)}
          \State \textbf{return} $pose$
        \EndIf
      \EndFor
      \State \textbf{return} null
    \EndProcedure
  \end{algorithmic}
\end{algorithm}


==> Algorithms/04-custom-observation-simple-compute01c1.tex <==
\begin{algorithm}[H]

  \caption{Subroutine for computing $c_{0}$ and $c_{1}$ if $c_{1}$ is not already valid.}

  \label{alg:04-custom-observation-simple-compute01c1}

  \begin{algorithmic}[1]

    \Procedure{COMPUTE-C0-C1}{$o$, $I$, $R$, $pushPose$, $c_{0}$, $c_{1}$}
      \State $c_{1} \gets \emptyset$
      \State $totalCost \gets +\infty$

      \For{each $obsPose$ in $o.obsPoses$}
        \State $c_{0_{cur}} \gets A$*($R$, $obsPose$, $I.occGrid$)
        \State $c_{1_{cur}} \gets A$*($obsPose$, $pushPose$, $I.occGrid$)
        \State $newTotalCost = |c_{0_{cur}}| + |c_{1_{cur}}|$
        \If{$newTotalCost < +\infty$ AND ($newTotalCost < totalCost$ OR ($newTotalCost = totalCost$ AND $|c_{0_{cur}}| < |c_{0}|$)}
          \State $c_{0} = c_{0_{cur}}$
          \State $c_{1} = c_{1_{cur}}$
          \State $totalCost = |c_{0}| + |c_{1}|$
        \EndIf
      \EndFor
    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/04-custom-observation-simple-planforobstacle.tex <==
\begin{algorithm}[H]

  \caption{Obstacle evaluation subroutine modified for allowing observation.}

  \label{alg:04-custom-observation-planforobstacle}

  \begin{algorithmic}[1]

    \Procedure{PLAN-FOR-OBSTACLE}{$o$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$}

      \If{$o \in blockedObsL$ \hlgreen{OR $o.movableStatus = IS\_NOT\_MOVABLE$}} \label{lst:line:identified_1}
        \State \textbf{return} null
      \EndIf

      \State $P_{o,d}$ $\gets \emptyset$
      % \State $BA \gets null$

      \For{each $pushPose$ in $o.pushPoses$}
        \State $pushUnit \gets (cos(pushPose.yaw), sin(pushPose.yaw))$

        \State $c_{1} \gets A$*($R$, $pushPose$, $I.occGrid$) \label{lst:line:c1_computation}

        \If{$c_{1} = \emptyset$}
          \State \textbf{continue}
        \EndIf

        %% BEGIN HLGREEN
        \State \hlgreen{$c_{0} \gets \emptyset$}

        \If{\hlgreen{$o.movableStatus = IS\_MAYBE\_MOVABLE$}} \label{lst:line:identified_2}

          \State \hlgreen{$obsPose \gets$ GET-FIRST-PATH-OBSPOSE($o$, $c_{1}$, $I$)} \label{lst:line:keep_c1_1}

          \If{\hlgreen{$obsPose \neq$ null}}
            \State \hlgreen{$c_{0}, c_{1} \gets c_{1}[c_{1}.firstPose:obsPose], c_{1}[obsPose:c_{1}.lastPose]$} \label{lst:line:keep_c1_2}
          \Else
            \State \hlgreen{COMPUTE-C0-C1($o$, $I$, $R$, $pushPose$, $c_{0}$, $c_{1}$)}

            \If{\hlgreen{$c_{0} = \emptyset$ OR $c_{1} = \emptyset$}} \label{lst:line:noc0c1_1}
              \State \hlgreen{\textbf{continue}}
            \EndIf \label{lst:line:noc0c1_2}
          \EndIf
        \EndIf
        %% STOP HLGREEN

        \State $seq \gets 1$

        \State $translation \gets pushUnit * onePushDist * seq$

        \State $safeSweptArea \gets $GET-SAFE-SWEPT-AREA($o$, $translation$, $I$)

        \State $oSimPose \gets pushPose + translation$

        \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$

        \State $C_{est} \gets ($\hlgreen{$(c_{0} \neq \emptyset ? |c_{0}| : 0)$}$ + |c_{1}| + |c_{3_{(Est)}}|) * moveCost + |translation| * o.pushCost$

        \While{$C_{est}$ $ \leq p_{opt}.cost$ AND $safeSweptArea \neq$ null}

          % \If{CHECK-NEW-OPENING($I.occGrid$, $o$, $translation$, $BA$)}
            \State $c_{2} \gets \{pushPose, oSimPose\}$
            \State $c_{3} \gets A$*($oSimPose$, $R_{goal}$, $I.withSimulatedObstacleMove$)
            \If{$c_{3} \neq \emptyset$}
              \State $p.components \gets$ \hlgreen{$c_{0} \neq \emptyset$ ? [$c_{0}$, $c_{1}$, $c_{2}$, $c_{3}$] : [$c_{1}$, $c_{2}$, $c_{3}$]}
              \State $p.cost \gets ($\hlgreen{$(c_{0} \neq \emptyset ? |c_{0}| : 0)$}$ + |c_{1}| + |c_{3}|) * moveCost + |c_{2}| * o.pushCost$
              \State $p.minCost \gets |c_{2}| * o.pushCost + |c_{3}| * moveCost$
              \State \dots \Comment{Affectation of other variables of $p$ (lines \ref{lst:line:ovaraffec1} to \ref{lst:line:ovaraffec2} in Algorithm \ref{alg:03-custom-basicmods-planforobstacle})}
            \EndIf
          % \EndIf

          \State $seq \gets seq + 1$

          \State $translation \gets pushUnit * onePushDist * seq$

          \State $safeSweptArea \gets $GET-SAFE-SWEPT-AREA($o$, $translation$, $I$)

          \State $oSimPose \gets pushPose + translation$

          \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$

          \State $C_{est} \gets ($\hlgreen{$(c_{0} \neq \emptyset ? |c_{0}| : 0)$}$ + |c_{1}| + |c_{3_{(Est)}}|) * moveCost + |translation| * o.pushCost$

        \EndWhile

      \EndFor

    \State \textbf{return} $p \in P_{o,d}$ with minimal $p.cost$ or null if $P_{o,d} = \emptyset$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/05-custom-placement-getocccost.tex <==
\begin{algorithm}[H]

  \caption{Obstacle placement cost evaluation subroutine.}

  \label{alg:05-custom-placement-getocccost}

  \begin{algorithmic}[1]

    \Procedure{GET-OCC-COST}{$simOccPoints$, $occCostGrid$}

      \State{$VALUE\_RANGE \gets (FORBIDDEN\_VALUE - ALLOWED\_VALUE)$}

      \State{$cost \gets 1$}

      \For{each $point$ in $simOccPoints$}
        \State $valueForPoint \gets occCostGrid[point]$
        \If{$valueForPoint = FORBIDDEN\_VALUE$} \label{lst:line:maxocccost_1}
          \State \textbf{return} $+\infty$ \label{lst:line:maxocccost_2}
        \ElsIf{$valueForPoint = ALLOWED\_VALUE$} \label{lst:line:noocccost_1}
          \State $valueForPoint \gets 0$
        \EndIf \label{lst:line:noocccost_2}
        \State{$cost \gets cost + valueForPoint / VALUE\_RANGE$} \label{lst:line:sumocccost}
      \EndFor

      \State \textbf{return} $cost$
    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/05-custom-placement-planforobstacle.tex <==
\begin{algorithm}[H]

  \caption{Obstacle evaluation subroutine modified for considering placement.}

  \label{alg:05-custom-placement-planforobstacle}

  \begin{algorithmic}[1]

    \Procedure{PLAN-FOR-OBSTACLE}{$o$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$, $occCostGrid$}

      \State \dots \Comment{Initialization (lines \ref{lst:line:initobs1} to \ref{lst:line:initobs2} in Algorithm \ref{alg:03-custom-basicmods-planforobstacle})}

      \For{each $pushPose$ in $o.pushPoses$}
        \State \dots \Comment{Loop initialization (lines \ref{lst:line:loop1} to \ref{lst:line:loop2} in Algorithm \ref{alg:03-custom-basicmods-planforobstacle})}

        \State \hlgreen{$suppC_{M} \gets $GET-OCC-COST(GET-OBS-POINTS($o$, $translation$), $occCostGrid$)}

        \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$

        \State $C_{est} \gets (|c_{1}| + |c_{3_{(Est)}}|) * moveCost + |translation| * o.pushCost *$ \hlgreen{$suppC_{M}$}

        \While{$C_{est}$ $ \leq p_{opt}.cost$ AND $safeSweptArea \neq$ null}

          % \If{CHECK-NEW-OPENING($I.occGrid$, $o$, $translation$, $BA$)}
            \State $c_{2} \gets \{pushPose, oSimPose\}$
            \State $c_{3} \gets A$*($oSimPose$, $R_{goal}$, $I.withSimulatedObstacleMove$)
            \If{$c_{3} \neq \emptyset$}
              \State $p.components \gets$ [$c_{1}$, $c_{2}$, $c_{3}$]
              \State $p.cost \gets (|c_{1}| + |c_{3}|) * moveCost + |c_{2}| * o.pushCost *$ \hlgreen{$suppC_{M}$}
              \State $p.minCost \gets |c_{2}| * o.pushCost *$ \hlgreen{$suppC_{M}$} $+ |c_{3}| * moveCost$
              \State \dots \Comment{Affectation of other variables of $p$ (lines \ref{lst:line:ovaraffec1} to \ref{lst:line:ovaraffec2} in Algorithm \ref{alg:03-custom-basicmods-planforobstacle})}
            \EndIf
          % \EndIf

          \State \dots \Comment{Loop variable update (lines \ref{lst:line:loopvarup1} to \ref{lst:line:loopvarup2} in Algorithm \ref{alg:03-custom-basicmods-planforobstacle})}

          \State \hlgreen{$suppC_{M} \gets $GET-OCC-COST(GET-OBS-POINTS($o$, $translation$), $occCostGrid$)}

          \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$

          \State $C_{est} \gets (|c_{1}| + |c_{3_{(Est)}}|) * moveCost + |translation| * o.pushCost *$ \hlgreen{$suppC_{M}$}

        \EndWhile

      \EndFor

    \State \textbf{return} $p \in P_{o,d}$ with minimal $p.cost$ or null if $P_{o,d} = \emptyset$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/06-custom-dynamic-makeandexecuteplan.tex <==
\begin{algorithm}[H]

  \caption{Execution loop taking dynamic obstacles into account.}

  \label{alg:06-custom-dynamic-makeandexecuteplan}

  \begin{algorithmic}[1]

    \Procedure{MAKE-AND-EXECUTE-PLAN}{$R_{init}$, $R_{goal}$, $I_{init}$}

      \State \dots \Comment{Initialization (lines \ref{lst:line:initbis1} to \ref{lst:line:initbis2} in Algorithm \ref{alg:03-custom-basicmods-makeandexecuteplan})}

      \State $isObsMoved \gets False$

      \While{$R \neq R_{goal}$}

        \State UPDATE-FROM-NEW-INFORMATION($I$)

        \If{$I$.freeSpaceCreated}
          \State $minCostL \gets \emptyset$
        \EndIf

        \State $\mathcal{O} \gets I.allObstacles$

        \State $isPlanNotColliding \gets p_{opt} \bigcap \mathcal{O} \neq \emptyset$

        \State \hlgreen{$isObsMoved \gets I.movedObstacles \neq \emptyset$}

        \State \dots \Comment{Plan validity checks (lines \ref{lst:line:validity1} to \ref{lst:line:validity2} in Algorithm \ref{alg:03-custom-basicmods-makeandexecuteplan})}

        \State \hlgreen{$isPlanValid \gets$ ($isPlanNotColliding$ AND $isManipSuccess$ AND $isManipSafe$ AND $isPushPoseValid$)}

        \If{\hlgreen{\textbf{not} $isPlanValid$}}
          \State $p_{opt}.components \gets$ [$A$*($R$, $R_{goal}$, $I.occGrid$)]
          \State $p_{opt}.cost \gets |p_{opt}| * moveCost$
        \EndIf
        \If{\hlgreen{\textbf{not} $isPlanValid$ OR ($isObsMoved$)}}
          \State MAKE-PLAN($R$, $R_{goal}$, $I$, $\mathcal{O}$, $blockedObsL$, $p_{opt}$, $euCostL$, $minCostL$)
          \State \hlgreen{$isManipSuccess \gets True$} \Comment{Line \ref{lst:line:ismanipsuccess} in Algorithm \ref{alg:02-levihn-makeandexecuteplan} is moved here.}
          \State \hlgreen{\textbf{continue}}
        \EndIf

        \State \dots \Comment{Execution (lines \ref{lst:line:exec1} to \ref{lst:line:exec1bis} and \ref{lst:line:exec2bis} to \ref{lst:line:exec2} in Algorithm \ref{alg:02-levihn-makeandexecuteplan})}
        \State \dots \Comment{Execution (lines \ref{lst:line:exec1} to \ref{lst:line:exec2} in Algorithm \ref{alg:02-levihn-makeandexecuteplan})}

      \EndWhile

      \State \textbf{return} $True$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/07-custom-merge-makeandexecuteplan.tex <==
\begin{algorithm}[H]

  \caption{Merged execution loop.}

  \label{alg:07-custom-merge-makeandexecuteplan-part1}

  \begin{algorithmic}[1]

    \Procedure{MAKE-AND-EXECUTE-PLAN}{$R_{init}$, $R_{goal}$, $I_{init}$}

      \State $R \gets R_{init}$
      \State $\mathcal{O}_{new} \gets \emptyset$
      \State $isManipSuccess \gets True$
      \State $blockedObsL \gets \emptyset$
      \State $euCostL, minCostL \gets \emptyset, \emptyset$

      \State $I \gets I_{init}$

      \State $p_{opt}.components \gets [$$A$*($R_{init}$, $R_{goal}$, $I.occGrid$)]
      \State $p_{opt}.cost \gets |p_{opt}| * moveCost$

      \State $isObservable \gets True$

      \While{$R \neq R_{goal}$}

        \State UPDATE-FROM-NEW-INFORMATION($I$)

        \If{$I$.freeSpaceCreated}
          \State $minCostL \gets \emptyset$
        \EndIf

        \State $\mathcal{O}_{new} \gets \mathcal{O}_{new} \bigcup I.newObstacles$

        \State $\mathcal{O} \gets I.allObstacles$

        \State $isPlanNotColliding \gets p_{opt} \bigcap \mathcal{O}_{new} \neq \emptyset$

        \State $isBlockingObsMoved \gets I.movedObstacles \neq \emptyset$

        \State $isPushPoseValid \gets True$
        \State $isManipSafe \gets True$
        \State $isObstacleSame \gets True$
        \If{$p_{opt}.o$ exists}
          \State $isObstacleSame \gets \mathcal{O}[p_{opt}.o] = p_{opt}.o$
          \If{\textbf{not} $isObstacleSame$}
            \State $p_{opt}.o \gets \mathcal{O}[p_{opt}.o.id]$
            \State $p_{opt}.safeSweptArea \gets$ GET-SAFE-SWEPT-AREA($p_{opt}.o$, $p_{opt}.translation$, $I$)
            \If{$p_{opt}.nextStepComponent$ is $ c_{1}$ AND $p_{opt}.pushPose \not\in p_{opt}.o.pushPoses$}
              \State $isPushPoseValid \gets False$
            \EndIf
          \EndIf
          \If{$p_{opt}.safeSweptArea \bigcap \mathcal{O} \neq \emptyset$}
            \State $isManipSafe \gets False$
          \EndIf
        \EndIf

        \State $isPlanValid \gets$ ($isPlanNotColliding$ AND $isManipSuccess$ AND $isManipSafe$ AND $isPushPoseValid$ AND $isObservable$)

        \If{\textbf{not} $isPlanValid$}
          \State $p_{opt}.components \gets$ [$A$*($R$, $R_{goal}$, $I.occGrid$)]
          \State $p_{opt}.cost \gets |p_{opt}| * moveCost$
        \EndIf
        \If{\textbf{not} $isPlanValid$ OR ($isBlockingObsMoved$)}
          \State MAKE-PLAN($R$, $R_{goal}$, $I$, $\mathcal{O}$, $blockedObsL$, $p_{opt}$, $euCostL$, $minCostL$)
          \State $isManipSuccess \gets True$
          \State \textbf{continue}
        \EndIf

        \algstore{makeandexecuteplan_merge_store}

  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]

  \label{alg:07-custom-merge-makeandexecuteplan-part2}

  \begin{algorithmic}[1]

        \algrestore{makeandexecuteplan_merge_store}

        \If{$p_{opt}.components = \emptyset$}
          \State \textbf{return} $False$
        \EndIf

        \State $isManipSuccess \gets True$
        \State $isObservable \gets True$
        \State $R_{next} \gets p_{opt}$.getNextStep()
        \If{$p_{opt}.o \neq$ null $p_{opt}.o.movableStatus = IS\_MAYBE\_MOVABLE$ AND \textbf{not} $isObstacleSame$ AND ($c_{next} = c_{0}$ OR $c_{next} = c_{1}$)}
          \State $fObsPose \gets$ GET-FIRST-PATH-OBSPOSE($p_{opt}.o$, $p_{opt}$.get-$c_{0}$() + $p_{opt}$.get-$c_{1}$(), $I$)
          \If{$fObsPose =$ null}
            \State $isObservable \gets False$
            \State \textbf{continue}
          \EndIf
        \EndIf
        \State $R_{real} \gets$ ROBOT-GOTO($R_{next}$)
        \If{$p_{opt}.nextStepComponent$ is $c_{2}$ AND $R_{real} \neq R_{next}$}
          \State $isManipSuccess \gets False$
          \State $blockedObsL \gets blockedObsL \bigcup p_{opt}.o$
        \EndIf
        \State $R \gets R_{real}$

      \EndWhile

      \State \textbf{return} $True$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/07-custom-merge-optimized-planforobstacle.tex <==
\begin{algorithm}[H]

  \caption{Merged obstacle evaluation subroutine}

  \label{alg:07-custom-merge-optimized-planforobstacle-part1}

  \begin{algorithmic}[1]

    \Procedure{PLAN-FOR-OBSTACLE}{$o$, $p_{opt}$, $I$, $R$, $R_{goal}$, $blockedObsL$}

      \If{$o \in blockedObsL$ OR $o.movableStatus = IS\_NOT\_MOVABLE$}
        \State \textbf{return} null
      \EndIf

      \State $P_{o,d}$ $\gets \emptyset$
      % \State $BA \gets null$

      \For{each $pushPose$ in $o.pushPoses$}
        \State $pushUnit \gets (cos(pushPose.yaw), sin(pushPose.yaw))$

        \State $c_{1} \gets A$*($R$, $pushPose$, $I.occGrid$)

        \If{$c_{1} = \emptyset$}
          \State \textbf{continue}
        \EndIf

        \State $c_{0} \gets \emptyset$

        \If{$o.movableStatus = IS\_MAYBE\_MOVABLE$}

          \State $obsPose \gets$ GET-FIRST-PATH-OBSPOSE($o$, $c_{1}$, $I$)

          \If{$obsPose \neq$ null}
            \State $c_{0}, c_{1} \gets c_{1}[c_{1}.firstPose:obsPose], c_{1}[obsPose:c_{1}.lastPose]$
          \Else
            \State OPT-COMPUTE-C0-C1($o$, $I$, $R$, $pushPose$, $c_{0}$, $c_{1}$)

            \If{$c_{0} = \emptyset$ OR $c_{1} = \emptyset$}
              \State \textbf{continue}
            \EndIf
          \EndIf
        \EndIf

        \State $seq \gets 1$

        \State $translation \gets pushUnit * onePushDist * seq$

        \State $safeSweptArea \gets $GET-SAFE-SWEPT-AREA($o$, $translation$, $I$)

        \State $oSimPose \gets pushPose + translation$

        \State $suppC_{M} \gets $GET-OCC-COST(GET-OBS-POINTS($o$, $translation$), $occCostGrid$)

        \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$

        \State $C_{est} \gets ((c_{0} \neq \emptyset ? |c_{0}| : 0) + |c_{1}| + |c_{3_{(Est)}}|) * moveCost + |translation| * o.pushCost * suppC_{M}$

        \algstore{planforobstacle_merge_store}

  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]

  \label{alg:07-custom-merge-optimized-planforobstacle-part2}

  \begin{algorithmic}[1]

        \algrestore{planforobstacle_merge_store}

        \While{$C_{est}$ $ \leq p_{opt}.cost$ AND $safeSweptArea \neq$ null}

          % \If{CHECK-NEW-OPENING($I.occGrid$, $o$, $translation$, $BA$)}
            \State $c_{2} \gets \{pushPose, oSimPose\}$
            \State $c_{3} \gets A$*($oSimPose$, $R_{goal}$, $I.withSimulatedObstacleMove$)
            \If{$c_{3} \neq \emptyset$}
              \State $p.components \gets$ $c_{0} \neq \emptyset$ ? [$c_{0}$, $c_{1}$, $c_{2}$, $c_{3}$] : [$c_{1}$, $c_{2}$, $c_{3}$]
              \State $p.cost \gets ((c_{0} \neq \emptyset ? |c_{0}| : 0) + |c_{1}| + |c_{3}|) * moveCost + |c_{2}| * o.pushCost * suppC_{M}$
              \State $p.minCost \gets |c_{2}| * o.pushCost * suppC_{M} + |c_{3}| * moveCost$
              \State $p.o \gets$ COPY($o$)
              \State $p.translation \gets translation$
              \State $p.safeSweptArea \gets safeSweptArea$
              \State $p.pushPose \gets pushPose$
              \State $P_{o,d} \gets P_{o,d} \bigcup \{p\}$
              \If{$p.cost < p_{opt}.cost$}
                \State $p_{opt} \gets p$
              \EndIf
            \EndIf
          % \EndIf

          \State $seq \gets seq + 1$

          \State $translation \gets pushUnit * onePushDist * seq$

          \State $safeSweptArea \gets $GET-SAFE-SWEPT-AREA($o$, $translation$, $I$)

          \State $oSimPose \gets pushPose + translation$

          \State $suppC_{M} \gets $GET-OCC-COST(GET-OBS-POINTS($o$, $translation$), $occCostGrid$)

          \State $c_{3_{(Est)}} \gets \{oSimPose, R_{goal}\}$

          \State $C_{est} \gets ((c_{0} \neq \emptyset ? |c_{0}| : 0) + |c_{1}| + |c_{3_{(Est)}}|) * moveCost + |translation| * o.pushCost * suppC_{M}$

        \EndWhile

      \EndFor

    \State \textbf{return} $p \in P_{o,d}$ with minimal $p.cost$ or null if $P_{o,d} = \emptyset$

    \EndProcedure

  \end{algorithmic}
\end{algorithm}


==> Algorithms/app-01-opening-detection-part1.tex <==
\begin{algorithm}[H]

  \caption{Efficient Local Opening Detection algorithm, Levihn et. al. (2011), commented}

  \label{alg:opening_detection}

  \begin{algorithmic}[1]

    \Procedure{CHECK-NEW-OPENING}{$G$, $M_{i}$, $A_{M}$, $BA$}

      \State $M \gets$ GET-$M'_{i}$-MATRIX($M_{i}$) \Comment{\nameref{get_mi_matrix_note}}
      \State $x_{offset} \gets M_{i}.x$ \Comment{$M_{i}.x$ and $M_{i}.y$ are the map coordinates of $M_{i}$'s top left corner.}
      \State $y_{offset} \gets M_{i}.y$
      \If{$BA$ is null} \Comment{BA needs not be recomputed if the environment did not change.}
        \State $BA \gets$ GET-BLOCKING-AREAS($x_{offset}$, $y_{offset}$, $M$, $G$) \Comment{Blocking areas before manip.}
      \EndIf
      \State $x_{offset} \gets$ GET-NEW-X-POS($A_{M}$, $M_{i}$) \Comment{\nameref{x-y-pos_note}}
      \State $y_{offset} \gets$ GET-NEW-Y-POS($A_{M}$, $M_{i}$)
      \State $BA_{s} \gets$ GET-BLOCKING-AREAS($x_{offset}$, $y_{offset}$, $M$, $G$) \Comment{Blocking areas after manip.}
      \State $BA^*_{s} \gets [0][0](dim(M))$ \Comment{Since the window of $BA_{s}$ shifted with the manipulation of $M_{i}$, ...}

      \For{$k$ from 0 to $|BA^*_{s}|$} \Comment{... we shift it back for the future comparison with $BA$.}
        \For{$l$ from 0 to $|BA^*_{s}[i]|$}
          \State $x \gets (x_{offset} - M_{i}.x) + k$
          \State $y \gets (y_{offset} - M_{i}.y) + l$
          \If{$0 < x < |BA^*_{s}|$ AND $0 < y < |BA^*_{s}[x]|$}
            \State $BA^*_{s}[x][y] \gets |BA^*_{s}|[k][l]$
          \EndIf
        \EndFor
      \EndFor

      \State $Z \gets$ COMPARE($BA$, $BA^*_{s}$) \Comment{Finally, compare the two blocking aread configurations.}
      \If{$Z = [0][0](dim(M))$} \Comment{\nameref{interpreting_z_note}}
        \State return $false$
      \EndIf
      \State return $true$

    \EndProcedure

    \\

    \Procedure{GET-BLOCKING-AREAS}{$x_{off}$, $y_{off}$, $M$, $G$}

    \State $index \gets 1$
    \State $BA \gets [0][0](dim(M))$ \Comment{$[0][0](dim(M))$ represents the 0-Matrix of dimensions = $dim(M)$}

    \For{$x$ from 0 to $|M|$} \Comment{Iterate over $M$ to detect and tag blocking areas.}
      \For{$y$ from 0 to $|M[x]|$}
        \If{$M[x][y] \neq 0$ AND $G[x+x_{off}][y+y_{off}] \neq 0$} \Comment{\nameref{check_blockage_note}}
          \State ASSIGN-NR($BA$, $x$, $y$, $index$)  \Comment{$BA$ and $index$ are directly modified in the call.}
        \EndIf
      \EndFor
    \EndFor

    \State return $BA$ \Comment{Return the saved information on the blocked areas.}

    \EndProcedure

    \algstore{opening_detection}

  \end{algorithmic}

\end{algorithm}


==> Algorithms/app-02-opening-detection-part2.tex <==
\begin{algorithm}[H]
  \begin{algorithmic}[1]
    \algrestore{opening_detection}

    \Procedure{ASSIGN-NR}{$BA$, $x$, $y$, $index$}

    \For{$i$ from -1 to 1} \Comment{Assignment is performed based on the 3*3 neighborhood.}
      \For{$j$ from -1 to 1}
        \If{$BA[x+i][y+j] \neq 0$} \Comment{If a number is already in the neighborhood, ...}
          \State $BA[x][y] \gets BA[x+i][y+j]$ \Comment{... the same number is assigned to the element.}
          \State \textbf{return}
        \EndIf
      \EndFor
    \EndFor

    \State $BA[x][y] \gets index$ \Comment{Else a new number is assigned, equal to the new index.}
    \State $index \gets index + 1$ \Comment{Only increment index if new intersection is created.}
    \State \textbf{return}

    \EndProcedure

    \\

    \Procedure{COMPARE}{$BA$, $BA^*_{s}$} \Comment{This function checks for non-zero entries in both matrices.}

    \State $BS \gets$ COPY($BA$)
    \State $del_{num} \gets \emptyset$ \Comment{Set of the indexes of obstacles to delete from $BS$.}

    \For{$x$ from 0 to $|BS|$} \Comment{Iterate over $BS$.}
      \For{$y$ from 0 to $|BS[x]|$}
        \If{$BA[x][y] \in del_{num}$} \Comment{\nameref{deletion_note}}
          \State $BS[x][y] \gets 0$
        \EndIf
        \If{$BA[x][y] \neq 0$ AND $BA^*_{s}[x][y] \neq 0$} \Comment{\nameref{deletion_note}}
          \State $del_{num} = del_{num} \bigcup BS[x][y]$
          \State $BS[x][y] \gets 0$
        \EndIf
      \EndFor
    \EndFor

    \State \textbf{return} $BS$

    \EndProcedure

  \end{algorithmic}

\end{algorithm}

